What's color got to do with it? Face recognition in grayscale

State-of-the-art deep CNN face matchers are typically created using extensive training sets of color face images. Our study reveals that such matchers attain virtually identical accuracy when trained on either grayscale or color versions of the training set, even when the evaluation is done using color test images. Furthermore, we demonstrate that shallower models, lacking the capacity to model complex representations, rely more heavily on low-level features such as those associated with color. As a result, they display diminished accuracy when trained with grayscale images. We then consider possible causes for deeper CNN face matchers "not seeing color". Popular web-scraped face datasets actually have 30 to 60% of their identities with one or more grayscale images. We analyze whether this grayscale element in the training set impacts the accuracy achieved, and conclude that it does not. We demonstrate that using only grayscale images for both training and testing achieves accuracy comparable to that achieved using only color images for deeper models. This holds true for both real and synthetic training datasets. HSV color space, which separates chroma and luma information, does not improve the network's learning about color any more than in the RGB color space. We then show that the skin region of an individual's images in a web-scraped training set exhibits significant variation in their mapping to color space. This suggests that color carries limited identity-specific information. We also show that when the first convolution layer is restricted to a single filter, models learn a grayscale conversion filter and pass a grayscale version of the input color image to the next layer. Finally, we demonstrate that leveraging the lower per-image storage for grayscale to increase the number of images in the training set can improve accuracy of the face recognition model.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> tex_files/figures/rgb_vis.tex <==
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.45\textwidth]{results/rgb_vis/rgb_vis.drawio.png}
    \caption{\textbf{Identities with different skin tones tend to cluster in 3D RGB space}. From the figure, it is evident that the RGB representation of visible skin pixels for the same identity is not tightly clustered. This variation reflects the diverse nature of the training set, where individuals of the same identity can exhibit different skin tones depending on the lighting conditions. This observation suggests that color may not be a crucial piece of information for the network to utilize, given the considerable variation in skintones within the dataset for the same identity.}
    \label{fig:rgb_vis}
\end{figure}

==> tex_files/tables/class_accuracy.tex <==


\begin{table}[h!]
\centering
\resizebox{.5\columnwidth}{!}{%
\begin{tabular}{|c|ccc|}
\hline
Class        & RGB [\%]  & Gray [\%] & Error[\%]      \\  \hline
Beer Bottle         & $36$ & $66$ & $-30$      \\
Sports Car          & $54$ & $80$ & $-26$      \\
Cardigan            & $34$ & $60$ & $-26$      \\
Banister (Handrail) & $26$ & $50$ & $-24$      \\
Payphone            & $34$ & $56$ & $-22$      \\ \hline\hline
Frypan/skillet & $40$ & $40$ & $0$      \\
Moving Van & $66$ & $66$ & $0$      \\ \hline\hline
School Bus          & $88$ & $60$ & $28$       \\ 
Guacamole           & $56$ & $28$ & $28$       \\
LadyBug             & $82$ & $50$ & $32$       \\
Scorpion            & $62$ & $30$ & $32$       \\
Lemon               & $74$ & $24$ & $50$      \\ \hline
\end{tabular}
}
\vspace{0.2cm}

{\scriptsize $\Delta$  Difference of the accuracies computed as RGB - Gray }
\caption{Comparison of Accuracy Between RGB and Grayscale Images at the Class Level.}
\label{tab:class_accuracy}
\end{table}


==> tex_files/tables/general_vision.tex <==


\setlength\extrarowheight{2pt}
\begin{table}[h!]
\caption{Comparison of Accuracy for General Object Classification Tasks Using ResNets with RGB and Gray Images.}
\centering
\resizebox{.4\columnwidth}{!}{%
\begin{tabular}{|c|ccc|}
\hline
Network      & RGB [\%]     & Gray [\%]    & $\Delta$ [\%]  \\ \hline
Resnet-18    & 55.92 & 51.54 & 4.38 \\
ResNet-50    & 57.16 & 53.13 & 4.03 \\
ResNet-101   & 57.82 & 53.71  & 4.11  \\ \hline
\end{tabular}
}
\vspace{0.2cm}

{\scriptsize $\Delta$  Difference of accuracies computed as RGB - Gray }
\label{tab:general-vision}
\vspace{-1.5em}
\end{table}

